Mapping the Structure and Evolution of Software Testing Research Over the Past Three Decades

Background: The field of software testing is growing and rapidly-evolving. Aims: Based on keywords assigned to publications, we seek to identify predominant research topics and understand how they are connected and have evolved. Method: We apply co-word analysis to map the topology of testing research as a network where author-assigned keywords are connected by edges indicating co-occurrence in publications. Keywords are clustered based on edge density and frequency of connection. We examine the most popular keywords, summarize clusters into high-level research topics, examine how topics connect, and examine how the field is changing. Results: Testing research can be divided into 16 high-level topics and 18 subtopics. Creation guidance, automated test generation, evolution and maintenance, and test oracles have particularly strong connections to other topics, highlighting their multidisciplinary nature. Emerging keywords relate to web and mobile apps, machine learning, energy consumption, automated program repair and test generation, while emerging connections have formed between web apps, test oracles, and machine learning with many topics. Random and requirements-based testing show potential decline. Conclusions: Our observations, advice, and map data offer a deeper understanding of the field and inspiration regarding challenges and connections to explore.

==> old_results.tex <==
\iffalse 

\begin{figure}[!t]
    \centering
    \includegraphics[width=\textwidth]{Diagrams/countries.png}
    \caption{A visualization of collaboration between national research communities.}
    \label{fig:countries}
\end{figure}

\subsection{Collaboration Between National Research Communities}\label{sec:countries}

\begin{center}
\begin{framed}
Figure~\ref{fig:countries} illustrates how research communities of particular countries collaborate internationally. An interactive version of this map can be accessed by opening the \texttt{country20} files from the data package or at \url{https://greg4cr.github.io/other/2021-TestingTrends/countries.html}.
\end{framed}
\end{center}

\begin{figure}[!t]
    \centering
    \includegraphics[width=.9\textwidth]{Diagrams/topcountries.pdf} \vspace{-10pt}
    \caption{Percentage of the 49,802 sampled publications published by researchers in the top-contributing countries, along with average and median percentages of national research communities.}
    \label{fig:country_counts}
\end{figure}

In this map, we include all countries where researchers have published at least 20 publications in our sample. In total, our map contains 79 countries, grouped into six clusters. In Figure~\ref{fig:country_counts}, we list the ten counties whose communities have published the most publications. We also list the average and median percentage of publications published by national research communities. 

\begin{center} 
\begin{framed}
\textbf{RQ3 (International Collaboration):} The national research communities that have published the most publications are the United States (15,421 publications, or 30.97\% of the sample), China (6,430; 12.91\%), Germany (3,018; 6.06\%), India (2,550; 5.12\%), United Kingdom (2,272; 4.56\%), Italy (1,952; 3.92\%), Canada (1,925; 3.87\%), France (1,891; 3.80\%), Brazil (1,289; 2.59\%), and Japan (1,260; 2.53\%). 
\end{framed}
\end{center}

All ten of these national research communities have contributed over the average and median. The difference between average and median is influenced by the United States, which has contributed over twice as many publications as Chinese researchers---the second highest contributor. 

These countries are generally prosperous, with the necessary governance and economic conditions to have formed a viable software industry and academic programs in computer science or software engineering. These are countries where researchers have the opportunity to collaborate with local, national, or international researchers and software developers---and where those developers and researchers are willing and able to collaborate. 

To understand how these communities collaborate internationally, we can cluster countries according to the connections between the authors of the sampled publications. The distribution of countries into clusters is as follows:
\begin{itemize}
\setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt} 
    \item \textbf{Cluster 1:} Australia, Bangladesh, China, Hong Kong, India, Indonesia, Iraq, Japan, Lithuania, Malaysia, Nigeria, Philippines, Singapore, South Africa, South Korea, Sri Lanka, Taiwan, Thailand, USA, Vietnam
    \item \textbf{Cluster 2:} Belgium, Bulgaria, Croatia, Czech Republic, Denmark, Estonia, Finland, Germany, Hungary, Italy, Kazakhstan, Latvia, Poland, Portugal, Russia, Serbia, Slovakia, Slovenia, Switzerland, Ukraine
    \item \textbf{Cluster 3:} Algeria, Canada, Egypt, France, Iran, Jordan, Kuwait, Lebanon, Morocco, Oman, Pakistan, Qatar, Saudi Arabia, Tunisia, United Arab Emirates
    \item \textbf{Cluster 4:} Austria, Cyprus, Greece, Iceland, Ireland, Luxembourg, Netherlands, New Zealand, Norway, Romania, Sweden, Turkey, United Kingdom
    \item \textbf{Cluster 5:} Argentina, Brazil, Chile, Colombia, Costa Rica, Ecuador, Mexico, Peru, Spain, Uruguay
    \item \textbf{Cluster 6:} Israel
\end{itemize}
\noindent Before we detail our observations on collaboration patterns, it is worth noting that---like with research topics---a cluster does not solely determine the collaborators of researchers in particular countries. Consider, for example, France in Cluster 3. Researchers in France do not solely collaborate with researchers in the other countries in Cluster 3---in fact, they collaborate with every other cluster. However, France and the other national research communities in Cluster 3 do collaborate disproportionately, resulting in their grouping as a distinct cluster. 

\begin{figure}[!t]
\centering
\includegraphics[width=0.6\textwidth]{Diagrams/france.png} 
  \caption{Interactions between France and other Cluster 3 countries.}\label{fig:countries_france} 
\end{figure}
  
\begin{figure}[!t]
\centering
\includegraphics[width=0.9\textwidth]{Diagrams/iran.png}
  \caption{Interactions between Iran and other countries.}\label{fig:countries_iran} 
\end{figure}
    
\begin{figure}[!t]
\centering
\includegraphics[width=0.85\textwidth]{Diagrams/israel.png} 
  \caption{Interactions between Israel and other countries.}\label{fig:countries_israel}
\end{figure}

Examining Figure~\ref{fig:countries} and the list of countries immediately reveals that \textit{researchers tend to interact with researchers in their immediate geographic neighborhood}. This trend can be seen within a majority of the clusters. Cluster 1 contains a large number of countries in central or southern Asia or its surroundings, such as China, India, and Vietnam. Cluster 2 contains several European nations, with a focus on eastern Europe. Cluster 3 contains several Middle Eastern countries. Cluster 4 largely contains western Europe nations. Finally, Cluster 5 is largely focused on South and Central America.

This is a natural result. Universities and industry in neighboring countries may have shared interests, historical or cultural connections, and greater physical or temporal ease in collaborating on research. This was particularly true before the emergence of mature software support for remote meetings or asynchronous work in the past decade. In addition, researchers in smaller or less economically prosperous countries may find greater success in working with collaborators in nearby countries with larger or better-funded software industries and universities than they would in their local environment. 

Geographic neighborhood is not the sole determinant of collaboration patterns. For example, France falls into Cluster 3 and Spain falls into Cluster 5---while the rest of Europe is split across Clusters 2 and 4. This is also demonstrated by the United States not being clustered with its neighbors---Canada and Mexico---and Israel forming its own cluster. Other factors also influence how researchers collaborate internationally. 

Cluster 3, in particular, offers important lessons in how collaborations form. This cluster is largely focused on the Middle East and its immediate surroundings---containing countries such as Egypt, Iran, Saudi Arabia, and the United Arab Emirates. Many of these countries are geographic neighbors, but there are also some notable \textit{inclusions} to this cluster that are not part of the geographic neighborhood---France and Canada---and specific \textit{exclusions} that are illustrative.

France and Canada have strong \textit{cultural and linguistic ties}---particularly in Quebec, where French is the primary language. While the sampled articles were written in English, this cultural link may encourage collaboration for several reasons. First, there may be \textit{strong ties between particular institutions} that provide explicit or implicit incentives to form collaborations. For example, two institutions may have a research partnership or student exchange programs. Second, cultural and linguistic ties may result in \textit{movement of researchers} between the two regions. For example, students have a tendency to go to particular countries when choosing where to complete a Ph.D or when they attain a post-doctoral or professor position. When these researchers move, they still maintain ties to their previous location---including their collaborators. 

Colonialism or other \textit{historic ties} also may influence research collaborations between countries. For example, France held direct control or influence over Algeria, Egypt, Morocco, and other countries in Cluster 3. Even though this is no longer the case today, this historical connection may influence collaboration today---for instance, leading to institutional connections or influencing patterns movement of individual researchers. This can be seen from the interactions between France and other Cluster 3 countries in Figure~\ref{fig:countries_france}. A observation can also be made from the inclusion of Spain in Cluster 5---a cluster largely focusing on South or Central American nations. Spain held many of these countries as colonies, leading to lasting linguistic and cultural ties that still influence patterns of collaboration and movement today. 

\textit{Political factors} also influence how and when researchers collaborate. For example, legal restrictions in the United States and in Europe constrain collaboration with Iran. As a result, the western nation that Iranian researcher collaborate the most with is Canada. Canada is a common country for Iranians to move to for their graduate education~\cite{Basiri20:Canada}, and the connections they build may result in long-term collaborations between researchers in the two countries. Notably, Iranian researchers also \textit{do not} tend to collaborate with many of their geographic neighbors in Cluster 3, such as the United Arab Emirates or Saudi Arabia (see Figure~\ref{fig:countries_iran}). This may reflect the political and cultural divide within the region. 

Political factors also may explain why two geographic neighbors are specifically excluded from Cluster 3---Iraq and Israel. Israel, in particular, appears as its own ``cluster'', as it cannot be grouped with any of the other clusters (see Figure~\ref{fig:countries_israel}). Israel has a contentious political relationship with its geographic neighbors, and this is reflected in the collaborations of researchers in Israel with those in other nations. Israeli researchers interact with French and Canadian researchers, but not with those in any of the Middle Eastern nations. Israeli researchers also work with those in a variety of other countries, but those collaborations span across all clusters and not disproportionately with any one cluster. As a result, Israel forms its own cluster. 

Iraq also does not appear in Cluster 3 with other Middle Eastern nations. Rather, it appears in Cluster 1 due to its connections with the United States, Australia, and Malaysia. The unstable political situation in Iraq and the role of the United States in the country may influence the resulting research collaborations. For example, the Iraqi government offers a large number of scholarships for students to attend graduate school in the United States~\cite{Madhani12:Iraq}, influencing the movement of researchers.

\begin{center}
\begin{framed}
\textbf{RQ3 (International Collaboration):} Collaborations between researchers in different countries are heavily influenced by the geographic neighborhood. However, cultural, historical, linguistic, and political connections also influence collaborations through their influence on the movement of researchers or by creating implicit or explicit incentives to collaborate.
\end{framed}
\end{center}

\subsubsection{Emerging International Collaborations}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\textwidth]{Diagrams/countries-historical.png}
    \caption{A visualization of collaboration between national research communities, colored by the average year of publication.}
    \label{fig:countries_historical}
\end{figure}

Figure~\ref{fig:countries_historical} presents the collaborations between national research communities, colored by the average year of publication. This allows us to examine which communities have begun to contribute more heavily to research in software testing in recent years. An interactive version of this map can be accessed by selecting the ``Overlay'' visualization after opening the \texttt{country20} map and network files in VOSviewer.

This visualization allows us to understand which areas of the world have seen recent growth in their contributions to software testing literature. We focus on the countries with an average year of publication within the past five years (June 2015 or later). This could indicate either the emergence of new national communities or the recent, rapid growth in productivity of existing communities. 

The countries that have emerged in this period include (marked with their cluster):
\begin{itemize}
\setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt} 
    \item \textbf{2017:} Indonesia, Philippines (1); Ecuador, Peru (5) 
    \item \textbf{2016:} Iraq, Vietnam (1); Kazakhstan (2); Morocco, Qatar (3); Colombia (5)
    \item \textbf{2015:} Bangladesh, Nigeria (1); Tunisia (3); Luxembourg (4); Costa Rica (5)
\end{itemize}

\begin{figure}[!t]
\centering
       \begin{subfigure}{.7\textwidth}
        \centering
\includegraphics[width=\textwidth]{Diagrams/ecuador.png}
  \caption{Interactions between Ecuador and others.}
    \end{subfigure}%

       \begin{subfigure}{\textwidth}
        \centering
\includegraphics[width=\textwidth]{Diagrams/peru.png} 
  \caption{Interactions between Peru and other countries.}
    \end{subfigure}%
      \caption{Illustrations of historical country data to support our observations.} 
  \label{fig:countries_historical_observations} 
\end{figure}
    
    \begin{figure}[!t]
\centering
  \begin{subfigure}{.8\textwidth}
        \centering
\includegraphics[width=\textwidth]{Diagrams/indonesia.png}
  \caption{Interactions between Indonesia and others.}
    \end{subfigure}%

       \begin{subfigure}{.5\textwidth}
        \centering
\includegraphics[width=\textwidth]{Diagrams/luxembourg.png} 
  \caption{Luxembourg and Norway.} 
    \end{subfigure}%
  \caption{Additional illustrations of historical country data to support our observations.} 
  \label{fig:countries_historical_observations_2} 
\end{figure}


\iffalse 
\greg{to add: look at youngest clusters (most recent age of publication)}
Cluster 5 - 2014.86
Cluster 3 - 2014.8278
Cluster 1 - 2014.45
Cluster 2 - 2013.69
Cluster 4 - 2013.454
Cluster 6 - 2010.613 (just Israel) 
\fi

The primary areas of growth have been in Clusters 1 (in southeast Asia and Africa), 3 (Africa and the Middle East), and 5 (South America). In general, many of these countries are less economically developed than those in, e.g., Europe (Clusters 2 and 4). Their software industries and universities may not be as well established, or resources may not have been available for researchers until recent years. The emergence of these countries indicates that software testing research is not restricted to the highly-developed nations, and new perspectives from the researchers in these countries will expand the range of what is possible in testing research.

Researchers in emerging countries may collaborate with those in more established nations. For the South American countries in Cluster 5, there is some variance in who these partners are, but two are particularly common---Brazil and Spain. In South America, Brazil has a large and well-established community of software engineering researchers. As geographic neighbors, collaboration with this community may offer benefits. All four of the emerging South American countries speak Spanish as their primary language, and there are strong cultural and historic ties to Spain. This will naturally lead to collaboration. 

Researchers in Costa Rica and Peru (see Figure~\ref{fig:countries_historical_observations}(b) have strong collaborations with Brazil and Spain, as well as the United States and Canada. Researchers in Ecuador (see Figure~\ref{fig:countries_historical_observations}) have stronger ties to Europe, including Spain, France, and the United Kingdom. Researchers in Colombia collaborate widely, but there are strong ties to both Brazil and Spain. Researchers in the emerging nations in Cluster 1 tend to interact widely. However, collaboration with the United States, China, France, and the United Kingdom is common (for example, see Indonesia in Figure~\ref{fig:countries_historical_observations_2}(a)).

One entry that stands out in this list is Luxembourg, as the sole western European country in the emerging communities. Luxembourg is a small country. Its size means that even small changes in the research landscape can be easily observed. In 2012, Lionel Briand formed a research group at the International Centre for ICT Security, Reliability, and Trust at the University of Luxembourg, focused on software verification (among other topics). This group employs a relatively large number of researchers. Due to the productivity of this group, and the small size of the country, this research group has shifted the average publication date for software testing research from this country. This can further be seen in Figure~\ref{fig:countries_historical_observations_2}(b). Briand was formerly at the University of Oslo and Simula Research Lab in Norway, and maintained his collaborations after moving. As a result, there is a strong connection (note the thickness of the line) between Luxembourg and Norway. 

\begin{center}
\begin{framed}
\textbf{RQ4 (Emerging International Collaborations):} Research communities are emerging in southeast Asia, Africa, and South America. Researchers in these communities often collaborate with those in well-established countries (e.g., South American researchers often collaborate with Spanish researchers). 
\end{framed}
\end{center}

\iffalse

Any signs of decline in specific countries?

Older countries (removed those in top-10):

(probably just well-established, not declining)
118	australia	1.0005	0.0529	1	55	746	1127	12287	1781.1473	2011.6948	10.9024	1.5804
555	japan	0.7449	-0.284	1	52	590	1260	8127	1186.1725	2010.7627	6.45	0.9414
970	sweden	-0.0745	-0.5168	4	49	565	795	9527	1330.3455	2012.9421	11.9836	1.6734
403	finland	-0.629	-0.5055	2	41	323	426	3618	456.4549	2012.0704	8.493	1.0715

(potentially declining in interest/activity in software testing)
188	bulgaria	-0.2407	0.1066	2	29	61	66	236	31.4992	2012.9091	3.5758	0.4773
296	denmark	-0.3328	-0.2529	2	41	194	187	4658	601.0291	2012.738	24.9091	3.2141
486	hong kong	1.6621	-0.2686	1	26	277	324	6011	710.8831	2010.6883	18.5525	2.1941
537	ireland	0.1996	-0.3571	4	37	162	207	1863	260.2648	2012.9372	9	1.2573
544	israel	-0.77	-0.8302	6	29	187	292	2359	283.0403	2010.613	8.0788	0.9693
590	kuwait	0.5205	0.9699	3	14	30	52	237	29.5715	2012.0385	4.5577	0.5687
605	lebanon	0.5139	1.3183	3	9	27	81	667	60.7131	2012.0741	8.2346	0.7495
733	new zealand	0.2086	-0.5179	4	34	130	160	1918	225.7179	2012.8875	11.9875	1.4107
908	serbia	-0.4982	-0.0849	2	21	48	116	869	130.2927	2012.9741	7.4914	1.1232
929	slovenia	-0.4224	-0.3967	2	29	78	72	769	84.836	2012.0278	10.6806	1.1783
978	taiwan	0.637	-0.5675	1	34	157	592	4358	501.393	2011.5659	7.3615	0.8469

Hard to tell from average year alone whether something is fading in interest. Some indication from older average year + number of papers. 

I am somewhat more comfortable labeling research topics as "fading" than countries/institutions. It feels weird to say "Hong Kong is no longer as interested in software testing". It may be true, but it feels like more data is needed. Could check the dataset. When was the most recent paper published? Is there a clear downward trend?

Need to think some more about this. Much easier and "safer" to point out emerging nations than declining ones.
\fi

\begin{figure}[!t]
    \centering
    \includegraphics[width=\textwidth]{Diagrams/authors.png}
    \caption{A visualization of collaboration between authors.}
    \label{fig:authors}
\end{figure}

\subsection{Collaboration Between Researchers}\label{sec:authors}

The publications in our sample were written by researchers with a total of 462 unique names. It is likely that some researchers share a common name. For example, a small set of family names are very common in China. As a result, it is difficult to establish that a name belongs to a single researcher, especially as our data set spans decades of publications. Therefore, we will not state a list of the ``most prolific authors'', as we cannot ensure the accuracy of such a list. 

Instead, we are interested in using the \textit{connections between researchers} as a basis for making observations about collaboration patterns in software testing research. These 462 names have been grouped into 13 clusters. Examining these clusters reveals four primary factors that influence collaborations between researchers. The first two relate to factors that lead to the formation of \textit{clusters or sub-clusters of researchers}. The second two relate to factors that \textit{link those clusters and sub-clusters}. 

\begin{center}
\begin{framed}
Figure~\ref{fig:authors} illustrates the collaborations between researchers. An interactive version of this map can be accessed by opening the \texttt{authors20} files from the data package or at \url{https://greg4cr.github.io/other/2021-TestingTrends/authors.html}.
\end{framed}
\end{center}

\smallskip\noindent\textbf{Researchers collaborate heavily with other local researchers:} The first cluster---by far the largest---is almost entirely made up of authors with traditional Chinese and Korean names. We make two observations about this cluster. First, this cluster illustrates the natural allure of local connections. China is a very large country with many universities and a well-established software industry. Researchers in China have many opportunities to collaborate without stepping outside of their local borders. South Korea is located just outside of this border, and also has well-established research programs, which also makes collaboration likely.

Second, although Chinese researchers have been conducting software engineering research since the 1980s, their community was largely self-contained before ICSE---a major SE venue---was held in China in 2006~\cite{Mei06:China,Mei18:China}. Researchers in Cluster 1 certainly collaborate outside of their cluster. However, Chinese authors largely started publishing in top testing venues only in the past 15 years~\cite{Mei18:China}. Before this point, researchers in China primarily worked with other Chinese researchers, often within their own university~\cite{Mei06:China}. Outside collaboration is a relatively recent---though, now fast-growing---phenomenon. 

Many of the other clusters also show that researchers tend to collaborate locally. Many of the researchers in Cluster 2, for example, are located in northern Europe. As we can better ensure the uniqueness of researcher names, we can also observe that this cluster contains small sub-clusters of researchers from individual institutions and research groups within those institutions in northern Europe. Among others, these institutions include the University of Luxembourg (e.g., Lionel Briand, Mike Papadakis), Chalmers and the University of Gothenburg (e.g., Robert Feldt, Richard Torkar), Delft University of Technology (e.g., Arie van Deursen, Annibale Panichella), KTH Royal Institute of Technology (e.g, Martin Monperrus, Benoit Baudry), and Simula Research Lab (e.g., Shaukat Ali). 

Many of these institutions are located in a small physical range (Luxembourg, Netherlands, Norway, and Sweden), making collaboration easier. These particular institutions also have \textit{large research groups} dedicated to software testing. The researchers in these groups will naturally collaborate to accomplish goals that could not be accomplished alone. It is simpler to work with local researchers than to collaborate across the world. It is even simpler to collaborate locally. Almost all of the researchers in this cluster have collaborations outside of this cluster. However, it is natural that they would collaborate at a heavier rate locally. 

Similar observations are clear in many of the other clusters. Particular geographic areas (United Kingdom, Italy) and research groups can be again seen in Cluster 3, e.g., the University of Sheffield (Phil McMinn, Rob Hierons, Gordon Fraser---who recently moved to the University of Passau, and Jose Migeul Rojas---who recently moved to the University of Leicester). Many of the researchers in Cluster 4 are South Korean. In particular, many are located at the Korea Advanced Institute of Science and Technology (KAIST), which is a major contributor to software testing research. While researchers collaborate across the planet, natural clusters will form at a local level, depending on the density of testing researchers---i.e., within the local institution, the national community, or across neighboring nations. 

\smallskip\noindent\textbf{Researchers collaborate in particular topic areas:} The primary linking factor for many of the researchers in Cluster 3 is a particular research topic---search-based software testing. Most of these researchers also work on other topics, but search-based software testing is their primary focus area. They collaborate with other researchers on this topic heavily enough to form a distinct collaboration cluster. 

Strong sub-communities can form within the broader research community around topics that are sufficiently popular if efforts are made to create an environment that fosters collaboration. Search-based software engineering is such a community. Prominent researchers in this community have created specialized workshops and meeting venues to discuss challenges, including the Symposium on Search-Based Software Engineering, the International Workshop on Search-Based Software Testing, and the Crest Open Workshops at University College London. The growth of interest in this research area can at least be partially attributed to the dedication of the members of the community to collaborating with each other and organizing dedicated events on the topic. 

\begin{center}
\begin{framed}
\textbf{RQ3 (International Collaboration):} Researchers tend to collaborate heavily with others in their own institution, national community, or in nearby countries. They also collaborate heavily on particular research topics, encouraged by community-building efforts such as dedicated workshops. 
\end{framed}
\end{center}

\begin{figure}[!t]
\centering
       \begin{subfigure}{0.9\textwidth}
        \centering
\includegraphics[width=\textwidth]{Diagrams/briand.png}
  \caption{Interactions between Lionel Briand and others.}
    \end{subfigure}%

       \begin{subfigure}{\textwidth}
        \centering
\includegraphics[width=\textwidth]{Diagrams/annibale.png} 
  \caption{Interactions between Annibale Panichella and others.}
    \end{subfigure}%
      \caption{Illustrations of the movement of researchers in Cluster 2.} 
  \label{fig:authors_movement} 
\end{figure}

\smallskip\noindent\textbf{The movement of researchers forges connections across borders:} The institutional sub-clusters in Cluster 2 are linked not purely by the convenience of working with their geographic neighbors, but by the movement of researchers. As noted earlier, Lionel Briand moved from Simula to the University of Luxembourg. This connection can be seen in this cluster by the connection between both institutions through Briand (see Figure~\ref{fig:authors_movement}(a)). Similarly, Annibale Panichella was a post-doctoral researcher in Luxembourg before taking a position in Delft. That move can be seen in this cluster as well, in Figure~\ref{fig:authors_movement}(b). In most cases, these collaborations do not end with the movement of the researcher. They continue even as new, local collaborations form. Movement of researchers is a clear factor in the formation of collaborations. The ease of movement between countries in the European Union may help increase collaboration across borders, and not just institutions within a single nation. 

\begin{figure}[!t]
\centering
\includegraphics[width=0.9\textwidth]{Diagrams/rothermel.png}
      \caption{Interactions between Gregg Rothermel and others.} 
  \label{fig:authors_rothermel} 
\end{figure}

\smallskip\noindent\textbf{Prolific researchers link sub-clusters of researchers together:} As noted, many of the researchers in Cluster 5 are located at KAIST in South Korea. The others in this cluster are largely from the United States. The connecting link is Gregg Rothermel, a prolific researcher. Rothermel has a history of collaboration with KAIST. He was a visiting professor at KAIST in 2011 and maintains research collaborations with researchers at the institution. In turn, many of the researchers in this cluster are linked through collaboration with Rothermel, as illustrated in Figure~\ref{fig:authors_rothermel}. Others are linked indirectly by their associations with Mary Jean Harrold, who was also a major testing researcher and the Ph.D. supervisor of Rothermel. Similar connections can be seen throughout this network of researchers. For example, a major connecting point between disparate sub-clusters in Cluster 6 is Myra Cohen. 

Prolific researchers in software testing tend to collaborate with a large number of people, across the world. Naturally, then, these individuals are a connecting factor across otherwise separate communities. Such researchers can serve as a natural ``matchmaker'', helping to foster new collaborations within the field. 

\begin{center}
\begin{framed}
\textbf{RQ3 (International Collaboration):} Connections between localized clusters or sub-clusters of researchers are formed through the movement of researchers and through the collaborations of prolific researchers. 
\end{framed}
\end{center}
\fi 


